TADA! Text to Animatable Digital Avatars

We introduce TADA, a simple-yet-effective approach that takes textual descriptions and produces expressive 3D avatars with high-quality geometry and lifelike textures, that can be animated and rendered with traditional graphics pipelines. Existing text-based character generation methods are limited in terms of geometry and texture quality, and cannot be realistically animated due to inconsistent alignment between the geometry and the texture, particularly in the face region. To overcome these limitations, TADA leverages the synergy of a 2D diffusion model and an animatable parametric body model. Specifically, we derive an optimizable high-resolution body model from SMPL-X with 3D displacements and a texture map, and use hierarchical rendering with score distillation sampling (SDS) to create high-quality, detailed, holistic 3D avatars from text. To ensure alignment between the geometry and texture, we render normals and RGB images of the generated character and exploit their latent embeddings in the SDS training process. We further introduce various expression parameters to deform the generated character during training, ensuring that the semantics of our generated character remain consistent with the original SMPL-X model, resulting in an animatable character. Comprehensive evaluations demonstrate that TADA significantly surpasses existing approaches on both qualitative and quantitative measures. TADA enables creation of large-scale digital character assets that are ready for animation and rendering, while also being easily editable through natural language. The code will be public for research purposes.

==> figtex/06_failure_cases.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figs/failure-cases.pdf}  
\vspace{-2.0 em}
\caption{Failure cases on loose clothes and rough-textured fabric. }
\label{fig:failure_cases}
% \vspace*{-1. em} 
\end{figure} 

==> figtex/13_ablation_head_zoomin.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figs/ablation_head_zoomin.pdf}   
\vspace*{-2. em} 
\caption{Ablation study on head zoom in. We compare the qualitative results with prompt "\textit{Chef}" in two designed methods: one samples body cameras exclusively (\ie w/o zoom in), while the other samples both body and head cameras (\ie w/ zoom in).}
\label{fig:ablation_head_zoomin}
% \vspace*{-1. em} 
\end{figure} 
 

==> paper/_Ablation.tex <==
\paragraph{Hybrid representation and hierarchical rendering.}


\input{figtex/12_ablation_decoupling}
\noindent \textbf{Identity and Outfit Decoupling.} Customized prompts often involve more complex and specific requirements, making it challenging to achieve the same level of fidelity and accuracy as with iconic characters. While prompts for iconic characters which are simple and easy to optimize, customized prompts can lead to a degradation in performance, particularly in the facial area. This is because the face holds significant identity-related information compared to clothing descriptions, which introduce noise when optimizing face. To address this problem, \modelname intelligently decouples the identity and clothing aspects, utilizing identical information to learn high-quality head representations. This innovative approach leads to a remarkable enhancement in the quality of the generated results. \Fref{fig:ablation_decouple} visually presents two compelling examples that further demonstrate the effectiveness of this decoupling strategy in our framework.
  
\noindent \textbf{Near Head Sampling.} To capture high-quality facial details, \modelname employs a carefully designed camera sampling strategy that involves zooming in around the head. This deliberate approach empowers our framework to capture highly detailed, lifelike faces with exceptional fidelity.  
\input{figtex/13_ablation_head_zoomin}
 
 
